Exploring the Limits of Complexity: A Survey of Empirical Studies on Graph Visualisation

For decades, researchers in information visualisation and graph drawing have focused on developing techniques for the layout and display of very large and complex networks. Experiments involving human participants have also explored the readability of different styles of layout and representations for such networks. In both bodies of literature, networks are frequently referred to as being 'large' or 'complex', yet these terms are relative. From a human-centred, experiment point-of-view, what constitutes 'large' (for example) depends on several factors, such as data complexity, visual complexity, and the technology used. In this paper, we survey the literature on human-centred experiments to understand how, in practice, different features and characteristics of node-link diagrams affect visual complexity.

==> sections/charts.tex <==
%!TEX root = ../main.tex 
\section{Charts}

HP - I know that there are lots of ways that the data can be depicted – we need to be sure we make good choices. Trends over time are typically better represented by line charts (so, fig8 would be better as a line chart, I think); box charts for min/max/median/quartiles etc. I know that the interactive graphs allow us to identify each data point – but will not be possible in the paper. I found the representations of min and max in figs 2 and 3 confusing

\subsection{Graph Size}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/size-venue.pdf}
\caption{\label{fig:size-venue} graph size vs. Venue}
\end{figure}

\subsubsection{min and max number of edges vs number of nodes used in studies}


\move{

\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{figures/charts/graph-sizes.pdf}
\caption{\label{fig:graphsizes} The size of graphs used in user studies. The x-axis shows the number of nodes, while the y-axis shows the number of edges. Both axes have a log scale. The blue circles represent static graphs. The red show dynamic graphs. While the yellow and green circles show dynamic graphs with two slices and static graphs with dynamic attributes respectively.  The links between the nodes connect different graph sizes used in the same study.}
\end{figure*}

SD - While for static graphs the number of nodes increased from 10-20 in 1995 to several thousand 20 years later, the graph size of dynamic graphs stayed below 100 (with one exception in 2015). 

HP -  I think that we should initially focus on ‘studies’ rather than ‘papers’, since each study is an experiment in its own right – in fact, the only time we need to consider ‘papers’ is when we consider publication venues. I don’t even think that the fact that a study appeared in a paper with another study is important in the basic analysis – so, for example, I don’t think that the lines in fig 1 are useful or necessary.

DA - Agree with Helen here.  I think the yellow-red lines should be excluded (can't read them anyway).  However, the individual dots, I think, are very important.  If you want to distinguish min and max maybe select two different colours?  For print, can we make the individual dots smaller so we can see the glyphs?  Two scatterplots?

}

DA- Maybe list top ten experiments, by size, for static and dynamic experiments, look at the papers, and try to figure out how they were able to test such large graphs? 



\subsubsection{min and max number of nodes used in studies}

\move{

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graph-nodes.pdf}
\caption{\label{fig:graphnodes} graph nodes}
\end{figure}

\subsubsection{min and max number of edges used in studies}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graph-edges.pdf}
\caption{\label{fig:graphedges} graph edges}
\end{figure}



DA - We love graphs of about 100 nodes and about 50 nodes.  We also love min graphs of 50 nodes and 20 nodes.  Looks like at 2:1 of min to max.  No real trend seen in edge data other than low connectivity.  Looks like number of nodes is what people go for when selecting sizes.

TD - Yes! Further, it suggests people chose the number of nodes first, and then adjust the density to what is readable. 



\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/slices.pdf}
\caption{\label{fig:slices} Histogram of timeslices of dynamic graphs used. }
\end{figure}




DA - It would be interesting to produce a number of timeslices histogram for dynamic data.  I think that it won't show much, but it would be good to report we tried it.



}


%\caption{\label{fig:size-years} The order of graphs used in studies across time. Please note that a log scale is used for the y-axis. The Figure shows that studies conducted before 2006 did not use dynamic graphs. It also shows a change in the scope of graph sizes in recent years, where studies have been using graphs with fewer and more nodes.}

\subsubsection{Densities of min and max graph sizes used in studies}

\move{

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graph-density.pdf}
\caption{\label{fig:graphdensity} graph density}
\end{figure}

SD- How was the graph density computed? Formula? There exist different 
definitions in the literature. In particular, one can distinguish directed
and undirected graphs $\frac{|E|}{|V|(|V|-1)}$ vs.  $\frac{2|E|}{|V|(|V|-1)}$
VY - I used $\frac{2|E|}{|V|(|V|-1)}$. Is it enought if we highlight the type of graph (directed, undirected, tree, etc.) in the chart or should we measure the density differently, if we do does it become inconsistent?

DA - We could compute a single number, but I think this edge vs node plot is interesting enough.  Exponential trend.  Should we plot log/log?


\move{
SD - Not a single study dealt with very dense graphs. While the density decreases with graph size, the average node degrees ($\frac{2|E|}{|V|}$) fall within the band of 2 to 20 for almost all studies. 
}

DA - I think it might be good to list the top experiments here as well so that we can try to explain why the experiments were able to use such dense/large graphs.

TD - Dense graphs are mostly small < 100 nodes. Two studies mentioned matrix, edge compression.

}

\subsubsection{Static or Dynamic vs. Time}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graphtype-time.pdf}
\caption{\label{fig:graphtype-time} Number of studies according to static or dynamic graphs.}
\end{figure}


\subsubsection{Real or Generated vs. Time}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/realgen-time.pdf}
\caption{\label{fig:realgen-time} Number of studies by what kind of graphs they used.}
\end{figure}



\subsection{Tasks}

\subsubsection{Task Types per graph sizes}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graph-tasks.pdf}
\caption{\label{fig:graphtasks} The types of tasks performed within the studies and the size of the graphs used.}
\end{figure}

SD - With larger graph size the proportion of overview tasks increases while the proportion of topology tasks decreases.

DA - glyph size smaller?  Again, maybe top end of the chart we try and look at the studies there and explain why these types of tasks.

\subsubsection{Task Types along the years}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/year-tasks.pdf}
\caption{\label{fig:yeartasks} year tasks}
\end{figure}

\subsection{Interaction}

\subsubsection{Interaction Types per graph sizes}

HW - Graphs with nodes (>500) and edge (>2000?) always have interaction types
Hw- Create interaction happens only in small graphs (node < 20, edge < 100)

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/graph-interaction.pdf}
\caption{\label{fig:graphinteraction} The types of interaction used within the studies and the size of the graphs used.}
\end{figure}

\subsubsection{Interaction Types along the years}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/year-interaction.pdf}
\caption{\label{fig:yearinteraction} year interaction}
\end{figure}


%VY - The treemap for the different task types at different venues, does not show a lot of difference across venues. However the treemap for the interaction types at venues, has a lot of variation between the venues. E.g. GD has no interaction, while CHI has complex interaction types.

\subsection{Participants}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/year-participants.pdf}
\caption{\label{fig:yearparticipants} year participants}
\end{figure}

SD - For all CHI-papers the number of participants is below the average 
     of 50. 

DA - following that, most of the crowdsource/online studies (over 100 participants) seem to come from TVCG.
     
SD - The number of papers per year increased from 1 in the first decade (1995-2005) to 8 (2006-2016). Around 2005/2006 seems to be the turning point both with respect to the number of papers as well as the number of publication venues.

VY - In the meeting of July 7 TD noted that 2014 has a study with 788 participants. Could this be due to encouraging crowd sourcing? DA- this is a AMT study. 

DA - Interesting to note that first studies appear in GD (I think this is obvious), then Information Visualisation, and then this is followed by TVCG (well, TVCG versions of InfoVis papers).  Multivariate graphs?  Two studies and both in Information Visualisation.  For dynamic graphs, a similar thing happens with Diagrams is also there.  Smaller, more focused conferences/journals seem to break the early work first and the big conference/journals second? 



\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/year-participants-avg.pdf}
\caption{\label{fig:yearparticipantsavg} year participants average and median}
\end{figure}

DA - I don't think the average number is all that indicative.  There are average spikes for all years where there was a large crowdsourcing study .  Also the 2014 spike is artificial.  The inversion in the year 2000 is just because the majority of the studies were in one paper.  The median is probably better here.  

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/histo-participants.pdf}
\caption{\label{fig:histoparticipants} The frequency of number of participants, used in the controlled studies in our survey, shows that 76\% of the controlled studies use 40 or less participants.}
\end{figure}

DA - A number of interesting numbers pop out here. 12, 18, 28.  I seem to recall that some HCI researchers (don't have a citation) think that 12 is the minimum number of participants.  It would be interesting to see if many of the 12s are from HCI venues.  Also, we should check with an HCI researcher.  I don't know where 18 and 28 comes from...  

\subsection{Venue}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/year-venue.pdf}
\caption{\label{fig:yearvenue} The number of papers with empirical studies between 1995 and 2016.}
\end{figure}

VY - There is a significant rise in the number of papers in 2011. This could be due to changes in program committe members (as noted during the meeting of June 2 by HP). TVCG had four papers in 2008, but it dropped in 2009 and 2010 to rise back to four in 2011. GD and EuroVis had 1 paper each in 2010, but had 2 papers each in 2011. Inversely CHI had 1 paper in 2010, but none in 2011. Information Visualisation Journal had one paper as it would in years that it had a paper.

VY - CHI had one or two papers every other two years starting 2006. However since 2013, it has had a steady number of papers with a jump in 2016, where it holds the highest number of papers, double that of TVCG and its previous history.

SD - Number of papers with studies kicks off in 2005-2006. Number of papers before 2005 on average was 1. After 2006 it becomes 8.

\subsection{Number of Studies per Paper vs. Time}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/charts/studies-per-paper.pdf}
\caption{\label{fig:studies-per-paper} The number of empirical studies within a paper across the years between 1995 and 2016.}
\end{figure}

\section{Additional Charts}

HP -  It seems that there are a few different types of dimension:
 
(a)    Nature of graphs: size (nodes), size (edges), size (density), dynamic/static, real/fabricated
(b)    Nature of graph drawing: layout type/no layout
(c)    Nature of experiment: number of participants, task type, interaction type, within/between
(d)    Meta-analysis: venue of publication, date of publication
 
·        So, I think that we should report basic statistics for (a-c) as our starting point: a table of max, min, median, mean, for size, and \% of studies for the others – e.g. for task type, we would report the \% of studies that used each type of task. We might include some histograms (like fig 2) if they say something interesting. This basic statistical data will be interesting data in itself, before we look at correlations or trends.

Then, after this, we can look at interesting relationships between these values: e.g. number of participants vs density, interaction type vs number of nodes. At this stage, we are still simply looking at the set of studies.

  Then, we can look at the venues (in which case we look at ‘papers’ rather than ‘studies’) and trends for those dimensions that are interesting – personally, I am not sure that looking at the types of tasks by venue is particularly interesting (happy to be persuaded otherwise if anyone wants to argue….!), but number of participants by year definitely is.


